Learning and aggregating deep local descriptors for instance-level recognition

We propose an efficient method to learn deep local descriptors for instance-level recognition. The training only requires examples of positive and negative image pairs and is performed as metric learning of sum-pooled global image descriptors. At inference, the local descriptors are provided by the activations of internal components of the network. We demonstrate why such an approach learns local descriptors that work well for image similarity estimation with classical efficient match kernel methods. The experimental validation studies the trade-off between performance and memory requirements of the state-of-the-art image search approach based on match kernels. Compared to existing local descriptors, the proposed ones perform better in two instance-level recognition tasks and keep memory requirements lower. We experimentally show that global descriptors are not effective enough at large scale and that local descriptors are essential. We achieve state-of-the-art performance, in some cases even with a backbone network as small as ResNet18.

==> ext-plots.tex <==
\usepackage{tikzextern}
\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> fig/data.tex <==
\pgfplotstableread{
epoch loss std
1 0.18478 0.00004
2 0.18022 0.00037
3 0.16542 0.00015
4 0.15720 0.00073
5 0.15362 0.00050
6 0.14972 0.00056
7 0.14494 0.00045
8 0.14478 0.00026
9 0.14004 0.00027
10 0.13648 0.00019
11 0.13138 0.00019
12 0.12860 0.00022
13 0.12832 0.00051
14 0.12658 0.00028
15 0.12704 0.00008
16 0.12050 0.00017
17 0.11716 0.00021
18 0.12060 0.00022
19 0.11436 0.00033
20 0.11402 0.00027
}{\traincurvelossstd}

\pgfplotstableread{
epoch mAP std
0 39.970 0.000
5 59.046 0.259
10 61.972 0.214
15 63.880 0.362
20 64.702 0.152
}{\traincurveglobalstd}

\pgfplotstableread{
epoch mAP std
0 66.320 0.000
5 83.038 0.277
10 84.208 0.493
15 84.326 0.563
20 85.188 0.286
}{\traincurvelocalstd}



\pgfplotstableread{
n sco scostd mem memstd
400 81.58400 0.46727 118.39248 0.18482
600 83.78600 0.25081 168.49914 0.20172
800 84.87800 0.26955 216.79619 0.15851
1000 85.18800 0.28638 270.33898 9.35754
1200 85.43000 0.23917 310.21770 0.18190
1400 85.16400 0.18184 356.14185 0.29875
}{\redcurve}
\pgfplotstableread{
n sco scostd mem memstd
400 81.53000 0.27914 148.56938 0.19782
600 83.72600 0.17761 215.04011 0.17692
800 84.85800 0.17267 280.09461 0.27054
1000 85.31200 0.16654 344.35533 0.38659
1200 85.54600 0.19314 408.34484 0.55791
1400 85.21800 0.12156 471.99162 0.68796
}{\pinkcurve}
\pgfplotstableread{
n sco scostd mem memstd
400 81.13600 0.47179 148.69728 0.85295
600 83.51200 0.34638 215.84951 1.48910
800 84.09400 0.33856 281.69131 2.17711
1000 84.78000 0.16199 346.63217 2.86707
1200 84.80000 0.23091 411.03358 3.50180
1400 84.65600 0.08309 474.83144 4.14526
}{\yellowcurve}
\pgfplotstableread{
n sco scostd mem memstd
400 81.35800 0.27651 155.77868 1.27476
600 83.54600 0.30819 225.37282 1.48294
800 84.66600 0.29897 293.45440 1.73212
1000 85.14600 0.25555 360.53311 1.96054
1200 85.25200 0.23233 427.02866 2.21882
1400 84.87600 0.22861 492.87813 2.54401
}{\orangecurve}
\pgfplotstableread{
n sco scostd mem memstd
400 76.03200 0.50297 308.17286 0.84878
600 79.71800 0.61418 456.25675 1.17095
800 81.43800 0.49024 602.22177 1.37227
1000 82.68400 0.60065 746.43620 1.49513
1200 83.22800 0.62876 889.02945 1.47876
1400 83.84200 0.51207 1030.04818 1.49074
}{\magentacurve}
\pgfplotstableread{
n sco scostd mem memstd
400 79.27400 0.57441 233.24868 0.16322
600 82.16000 0.46613 337.34492 0.29383
800 83.95000 0.35287 437.33062 0.39826
1000 84.67600 0.36511 534.00844 0.52628
1200 85.31400 0.33613 627.91052 0.61201
1400 86.07800 0.35448 719.36905 0.64337
}{\greencurve}
\pgfplotstableread{
n sco scostd mem memstd
400 83.13400 0.36522 118.00969 0.56709
600 85.11400 0.33649 168.81768 0.77978
800 85.95400 0.43107 217.92269 1.13573
1000 86.86200 0.60529 265.92573 1.54574
1200 87.10600 0.44175 313.22532 1.90466
1400 87.17600 0.31954 360.03435 2.25650
}{\bluecurve}
\pgfplotstableread{
n sco scostd mem memstd
400 80.05400 0.22491 194.95923 0.28352
600 82.90200 0.11754 281.52904 0.41016
800 84.83800 0.15484 364.84234 0.44489
1000 86.18000 0.21863 443.11233 9.21084
1200 87.04200 0.24967 523.88451 0.62591
1400 87.68200 0.12221 600.26911 0.72663
}{\browncurve}


==> no-plots.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\extdata}[1]{}

